ASP-Core-2 Input Language Format

Standardization of solver input languages has been a main driver for the growth of several areas within knowledge representation and reasoning, fostering the exploitation in actual applications. In this document we present the ASP-Core-2 standard input language for Answer Set Programming, which has been adopted in ASP Competition events since 2013.

==> lex.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{EBNF Grammar and Lexical matching table}

\input{grammars}

\label{sec:lex}

\begin{small}
\begin{tt}
\begin{center}
\begin{longtable}{|l|l|l|}
\hline
 {\bf {\small Token Name}} & {\bf {\small Symbolic Value or} }         & {\bf {\small Lexical Value} }    \\
& {\bf {\small Symbolic Example} }  &\\
\hline
ID                  &$p$, $P$, q1, \dots                                         &  {\tt [A-Za-z][A-Za-z\_0-9]* \ }      \\
SYMBOLIC\_CONSTANT\  \  &$a$, $b$, $anna$, \dots                                     &  {\tt [a-z][A-Za-z\_0-9]*}      \\
VARIABLE            &$X$,$Y$, $Name:  $, \dots                                   &  {\tt [\_A-Z][A-Za-z\_0-9]*}    \\ \hline\hline
STRING              &\quo{http://bit.ly/cw6lDS}, \                               &  {\tt \textbackslash"[\^{}\textbackslash"*]\textbackslash"}\\
                    &\quo{Full name} , \dots & \\ \hline
ANON\_VAR           &\_                                                          &  {\tt "\_"}\\
       NUMBER       & 1, 0, 100000, \dots                                        & {\tt [0-9]+}\\
DOT                 &$.$                                                         &  {\tt "."}\\
BODY\_SEPARATOR     &$,$                                                         &  {\tt ","}\\
TERM\_SEPARATOR     &$,$                                                         &  {\tt ","}\\
QUERY\_MARK         &$?$                                                         &  {\tt "?"}\\
COLON               &$:$                                                         &  {\tt ":"}\\
HEAD\_SEPARATOR     &$\vee$                                                      &  {\tt "|" $|$ ";" $|$ "v"}\\
NEG                 &$-$                                                         &  {\tt "-" $|$ "\verb+~+"}\\
NAF                 &\naf                                                        &  {\tt "not"}\\
CONS                &$\leftarrow$                                                &  {\tt "<-" $|$ ":-"}\\ \hline \hline
PLUS                &$+$                                                         &  {\tt "+"}\\
MINUS               &$-$                                                         &  {\tt "-"}\\
TIMES               &$*$                                                         &  {\tt "*"}\\
DIV                 &$/$                                                         &  {\tt "/" $|$ "div"}\\
\hline
\hline
\hline
PARAM\_OPEN         &(                                                           &  {\tt "("}\\
PARAM\_CLOSE        &)                                                           &  {\tt ")"}\\
SQUARE\_OPEN        &$[$                                                         &  {\tt "["}\\
SQUARE\_CLOSE       &$]$                                                         &  {\tt "]"}\\
CURLY\_OPEN         &\{                                                          &  {\tt "\{"}\\
CURLY\_CLOSE        &\}                                                          &  {\tt "\}"}\\ \hline\hline
EQUAL               &$=$                                                         &  {\tt "=" $|$ "=="}\\
UNEQUAL             &$\not=$                                                     &  {\tt "<>" $|$ "!="}\\
LESS                &$<$                                                         &  {\tt "<"}\\
GREATER             &$>$                                                         &  {\tt ">"}\\
LESS\_OR\_EQ        &$\leq$                                                      &  {\tt "<="}\\
GREATER\_OR\_EQ     &$\geq$                                                      &  {\tt ">="}\\ \hline\hline
AGGR\_COUNT         &$\#count$                                                   &  {\tt "\#count"}\\
AGGR\_MAX           &$\#max$                                                     &  {\tt "\#max"}\\
AGGR\_MIN           &$\#min$                                                     &  {\tt "\#min"}\\
AGGR\_SUM           &$\#sum$                                                     &  {\tt "\#sum"}\\
\hline
 COMMENT  &  &  {\tt \verb+\%+.*\$}\\
 BLANK    &  &  {\tt [ \verb+\t+\verb+\n+]+} \\ \hline
\end{longtable}
\end{center}
\end{tt}
\end{small}

Lexical values are given in Flex\footnote{{\tt http://flex.sourceforge.net/}.} syntax.
The {\tt COMMENT} and {\tt BLANK} tokens can be freely interspersed amidst other tokens and have no
syntactical and semantic meaning.
